The Sufficiency of Off-Policyness and Soft Clipping: PPO is still Insufficient according to an Off-Policy Measure

The popular Proximal Policy Optimization (PPO) algorithm approximates the solution in a clipped policy space. Does there exist better policies outside of this space? By using a novel surrogate objective that employs the sigmoid function (which provides an interesting way of exploration), we found that the answer is ``YES'', and the better policies are in fact located very far from the clipped space. We show that PPO is insufficient in ``off-policyness'', according to an off-policy metric called DEON. Our algorithm explores in a much larger policy space than PPO, and it maximizes the Conservative Policy Iteration (CPI) objective better than PPO during training. To the best of our knowledge, all current PPO methods have the clipping operation and optimize in the clipped policy space. Our method is the first of this kind, which advances the understanding of CPI optimization and policy gradient methods. Code is available at https://github.com/raincchio/P3O.

==> ablation.tex <==



\subsection{Ablation Studies}
As the P3O objective has two parts, the sigmoidal preconditioner and the KL-divergence regularizer, we conducted an ablation study.
The following three variants were studied: \textbf{P3O-S} removes the sigmoidal preconditioner and replaces it with the identity mapping;  \textbf{P3O-K} removes the KL-divergence regularizer; \textbf{P3O-SK} removes both the preconditioner and KL-divergence, reducing to the TRPO objective. Figure \ref{fig:ablation} shows the performance of all these variants decreased sharply. Notably, P3O-K (with only the sigmoid preconditioning) outperforms P3O-S (with only the KL-divergence regularizer), showing that the sigmoid preconditioning is the primary driver of improvement in P3O. 
% The P3O with sigmoid preconditioning and the KL divergence regularizer performs the best, indicating that our strategy is effective.

\begin{figure}[t]
\centering
\includegraphics[width=0.98\columnwidth]{figure/ablation.pdf} 
\caption{Ablation studies. P3O-S removes the sigmoid preconditioner and P3O-K removes KL-divergence regularizer; while P3O-SK removes both, reducing to the TRPO objective.
This shows both factors are important to the performance of P3O; in addition, preconditioning contributes more than the regularization.  
}
\label{fig:ablation}
\end{figure}


==> related.tex <==

\section{Related Works}

In this section, we briefly review the related works from four aspects.

\paragraph{Convex optimization methods.} Some work has developed approaches that simplify the optimization problem of reinforcement learning into a convex optimization problem. In the paper~\citep{yao2008preconditioned}, a framework of policy evaluation algorithms called the preconditioned temporal difference (PTD) learning is introduced. And in the paper~\citep{li2016preconditioned,sappl2019deep}, they use the preconditioning for deep neural network effective training. DAPO~\citep{wang2019divergence} proved that the convex optimization method could be used in the reinforcement learning problem and include the Bregman divergence to ensure minor and safe policy updates with off-policy data. Euclidean distance and Kullback Leibler (KL) divergence are instances of Bregman divergence. MDPO~\citep{tomar2021mirror} adds a proximity term that restricts two consecutive policies to be close to each other to the common expected reward objective, iteratively updates the policy by approximately solving a trust-region problem.

\paragraph{Compute Hessian Matrix.} Recently, there are many methods to improve sample efficiency based on the Trust-region second-order gradient optimization algorithms~\citep{schulman2015trust,wu2017scalable}. These methods calculate the approximate Hessian matrix to find an ideal gradient. However, the computational cost is enormous, and the Hessian matrix is not tackled for complex neural networks. Although \citep{wu2017scalable} designed a particular neural network struct for simplifying computation, the network structure is not generalizable for complex application situations. 

\paragraph{Policy Approximation.} Several studies go deeper into the policy aprroximation in RL, one of the famuous, is the clipping mechanism of the PPO algorithm, which relies upon optimizing parametrized policies by heuristic method. In~\citep{wang2020truly}, they adopt a new clipping function to support a rollback behavior to restrict the ratio between the new policy and the old one. In the paper~\citep{ye2020mastering}, when the estimate of the advantage is negative, their dual-clip operator will result in a better performance of the policy.  In \citep{hsu2020revisiting}, they review the multiple failure modes of the PPO algorithm and use beta distribution instead of the Gaussian distribution to get better performance. However, this is not to improve the algorithm but to replace the structure more suitable for specific environments. These studies only analyzed the effects of the PPO's clip operation and did not put forward the theory to explain why the clipping is needed. For the estimation of $\eta(\pi)$ under a behavior policy $\Tilde{\pi}$, possible methods include Retrace~\citep{wang2016sample} providing an estimator of state-action value, and V-trace~\citep{espeholt2018impala} providing an estimator of state value. But that two methods also suffer from the estimation variance.

\paragraph{Off-Policy Method.} For value-based algorithms, sample efficiency has also been considered from the aspect of data usage. In the DQN \citep{mnih2015human} algorithm, a replay buffer for learning previous experiences is used to improve sample efficiency. In the double-DQN \citep{van2016deep}, the overestimation problem is eliminated by decoupling the two steps of target Q action selection and target Q calculation. The DDPG\citep{lillicrap2019continuous} is a deterministic policy gradient algorithm based on actor-critic, solving continuous action space tasks that DQN cannot solve. TD3\citep{fujimoto2018addressing} follows the idea of double-DQN, using two independent critics to prevent overestimation, but can only be used for environments with continuous action spaces. In the SAC\citep{haarnoja2018soft}, they introduce entropy into a deep reinforcement learning algorithm, which provides sample-efficient learning while retaining the benefits of entropy maximization.

Compared with the previous method, our method uses preconditioner to better deal with the infinite variance problem. Low-variance gradients make learning more efficient, allowing fixed step-sizes to be used, potentially reducing the overall number of steps needed to reach convergence and resulting in faster training. And we can guarantee monotonic policy improvement by cooperating with the KL divergence constraint. 


\section{Hyper-parameter}\label{ap:parameter}

The detailed hyper-parameter is shown in the Table~\ref{tab:atari_hyperparameters}.
\begin{table}
\centering
\begin{tabular}{lrr}
\toprule
Env(type)  & MuJoCo  &Atari  \\
\midrule
Horizon (T)       & 2048  & 256   \\
Adam stepsize   & $1 \times 10^{-4}$   &  $2.5 \times 10^{-4}$ \\
Num. epochs  & 10   & 4   \\
Minibatch size  & 64  & 4   \\
Discount ($\gamma$)  & 0.99 &0.99     \\
GAE parameter ($\lambda$)  & 0.95 & 0.95  \\
Number of actors & 1 & 8 \\
KL coeff.$\beta_{kl}$  & 1 &0.1 \\
Simga coeff.$\beta_s$ & 1 & 1 \\
VF coeff.  & 1 & 1\\
Entropy coeff.  & 0 & 0.01 \\
Temperature($\tau$) . & 4& 4\\
\bottomrule
\end{tabular}
\caption{hyper-parameters used for the MuJoCo 3 million timesteps benchmark and for the Atari 100 million time-steps benchmark}
% \caption{Mean final scores (last 100 episodes) of SCPO and Dual-clip PPO on Atari games after 10M timesteps.}
\label{tab:atari_hyperparameters}
\end{table}
